Identifying Emotions from Walking using Affective and Deep Features

We present a new data-driven model and algorithm to identify the perceived emotions of individuals based on their walking styles. Given an RGB video of an individual walking, we extract his/her walking gait in the form of a series of 3D poses. Our goal is to exploit the gait features to classify the emotional state of the human into one of four emotions: happy, sad, angry, or neutral. Our perceived emotion recognition approach uses deep features learned via LSTM on labeled emotion datasets. Furthermore, we combine these features with affective features computed from gaits using posture and movement cues. These features are classified using a Random Forest Classifier. We show that our mapping between the combined feature space and the perceived emotional state provides 80.07% accuracy in identifying the perceived emotions. In addition to classifying discrete categories of emotions, our algorithm also predicts the values of perceived valence and arousal from gaits. We also present an EWalk (Emotion Walk) dataset that consists of videos of walking individuals with gaits and labeled emotions. To the best of our knowledge, this is the first gait-based model to identify perceived emotions from videos of walking individuals.

==> 7_application.tex <==
\section{Application: Virtual Character Generation}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{images/Ryan.png}
  \caption{\textbf{Application}: Our gaits and their perceived emotion labels can be used to generate virtual characters with different emotions. We show a character that is generated using our approach to convey basic emotions: angry, happy, sad, and neutral.}
  \label{fig:ryan}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{images/ApplicationOverview.png}
  \caption{\textbf{Virtual Character Generation}: We provide an overview of our end-to-end approach for simulating virtual characters. We represent the behavioral state of the virtual characters in a Behavioral Finite State Machine (BFSM) and use it to control their behavior based on the state of the environment, which consists of static and dynamic obstacles. We use our perceived emotion prediction to generate gaits for the virtual characters based on their desired emotions.}
  \label{fig:ApplicationOverview}
\end{figure}

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/saliency.png}
%     \caption{\textbf{Saliency Maps}: We present the saliency maps for examples from each of the four emotion classes, as learned by the network for a single walk cycle. The maps show activations on the joints during the walk cycle. Black represents no activation and red represents high activation. For all the emotion classes, the hand, feet and head joints have high activations, implying that the network deems these joints to be more important for determining the class. Moreover, the activation values on these joints for a high arousal emotion (\textit{e.g.}, angry) are higher than those for a low arousal emotion (\textit{e.g.}, sad), implying the network learns that higher arousal emotions lead to more vigorous joint movements.}
%     \label{fig:saliency}
% \end{figure*}

\begin{figure*}[!ht]
    \centering
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/saliency_angry.png}
        \caption{Angry}
        \label{fig:sal_angry}
    \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/saliency_happy.png}
        \caption{Happy}
        \label{fig:sal_happy}
    \end{subfigure}
    % \begin{subfigure}[t]{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{images/saliency_neutral.png}
    %     \caption{Neutral}
    %     \label{fig:sal_neutral}
    % \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/saliency_sad.png}
        \caption{Sad}
        \label{fig:sal_sad}
    \end{subfigure}%
    \caption{\textbf{Saliency Maps}: We present the saliency maps for examples from each of the for emotion classes, as learned by the network for a single walk cycle. The maps show activations on the joints during the walk cycle. Black represents no activation and red represents high activation. For all the emotion classes, the hand, feet and head joints have high activations, implying that the network deems these joints to be more important for determining the class. Moreover, the activation values on these joints for a high arousal emotion (\textit{e.g.}, angry) are higher than those for a low arousal emotion (\textit{e.g.}, sad), implying the network learns that higher arousal emotions lead to more vigorous joint movements.}
    \label{fig:saliency}
\end{figure*}

In this section, we present an application of our method that generates virtual characters with given desired emotions (Figure~\ref{fig:ryan}). 

\subsection{Overview}
We provide an overview of our end-to-end approach to simulating virtual characters in Figure~\ref{fig:ApplicationOverview}. We assume that the environment consists of static and dynamic obstacles. At the start of the simulation, we initialize the environment state with positions and dimensions of the static obstacles and the current positions and velocities of the dynamic obstacles. We also initialize a Behavioral Finite State Machine (BFSM) based on the user input and the intended tasks. We set up a 3D model for each virtual character that is rigged using automatic rigging software and associate a hierarchical skeleton with appropriate joint values.





% We use the joints of this hierarchical skeleton to update the visualization of the agent. 
% of a user's friend or a celebrity with a positive impression. We choose these familiar 3D model for the FVA because according to psychology research familiarity increases friendliness.

% At runtime, we update the BFSM state according to the state of the environment and whether the FVA has completed the assigned tasks. Based on the updated state, a global planning step is used to compute the next intermediate goal position and configuration for the FVA. Next, we compute velocities for local navigation (if it needs to change location in the real world) and decide gaits, gestures, and gazing behaviors according to the BFSM state. We then update the joint positions and angles of the FVA's hierarchical skeleton using the computed gaits, gestures, and gazing features. We visualize the FVA using the selected 3D model in an AR device such as the Microsoft HoloLens. We describe these components in detail below.

\subsection{Behavioral Finite State Machine}
We represent the behavioral state of the virtual characters in a BFSM and use it to control their behaviors. At runtime, we consider the environment state and the context of the current task and update the state of the BFSM that determines the virtual characters' behavior. This state also computes a goal position for each virtual character.

\subsection{Global and Local Navigation}
If the goal positions of virtual characters are different from their current positions, then a navigation algorithm is used to compute the trajectories to the new positions. To provide collision-free navigation in the presence of obstacles or other virtual characters, we utilize the multi-agent simulation framework, \textit{Menge}~\cite{curtis2016menge}. In this framework, a global navigation step first breaks down the goal positions into intermediate goals that avoid collisions with the static obstacles in the environment. Next, a local navigation step uses a reciprocal collision avoidance (RVO) approach to avoid collisions with dynamic obstacles and provide navigation to the intermediate goals~\cite{van2011reciprocal}. 

In this approach, we represent each agent on the 2D ground plane and generate smooth, stable, collision-free velocities. RVO is an agent-based approach that computes a collision-free 2D velocity for an agent given its preferred velocity, time horizon ($t_{max}$), and current positions and velocities of the all virtual agents in the environment. In other words, it computes a velocity that can generate a collision-free trajectory at time $t_{max}$. We update the character's location in the virtual world according to this collision-free trajectory at each frame.

\subsection{Gait Generation}\label{sec:gaitGeneration}
In addition to the goal position for each virtual character, the BFSM state also determines the desired emotion that each virtual character must convey. To achieve this, we use our gait-based approach to identify the perceived emotion. For each virtual character, we obtain a set of gaits that correspond to the desired emotion using our gait dataset and associated labels. We choose one of the gaits from this set and use it to update the joint positions of the agent in the virtual world. The selection of a gait can be made according to many criteria (such as personality or preferred walking speed).

% In our current implementation, we choose the gait randomly.

% At runtime, for each agent, we take the desired emotion $e_{des}$ as input. We use the gait emotion association metric and obtain a set of gaits $GEA(e_{des})$ that correspond to the desired emotion. We choose one of the gaits $G_{des}$ from $GEA(e_{des})$ and update the joint positions of the agent in the virtual world using the joint positions from $G_{des}$. The selection of  $G_{des}$ from $GEA(e_{des})$ can be made according to many criteria (such as personality or preferred walking speed). In our current implementation, we choose the gait randomly.

% \subsection{Local Navigation using Expressive Features}
% For navigation, we represent each agent on the 2D ground plane and compute its collision-free velocity. We use a reciprocal velocity obstacle-based method, RVO, to generate smooth, stable, collision-free velocities~\cite{van2008reciprocal}. RVO is an agent-based approach that computes a collision-free 2D velocity of an agent given its preferred velocity, time horizon ($t_{max}$), and current positions and velocities of the all virtual agents in the environment. In other words, it computes a velocity that can generate a collision-free trajectory at time $t_{max}$.

% Based on the chosen gait $G_{des}$ for an agent $i$, we set the preferred speed of the agent as the speed of the gait $G_{des}$. The speed of the gait $v_{des}$ is computed as follows:
% \begin{eqnarray}
%     v_{des} = ||\vec{p(J_{root,\tau})} - \vec{p(J_{root,0})}||/\tau,
% \end{eqnarray}
% where $\vec{p(J_{root,\tau})}$ and $\vec{p(J_{root,0})}$ represent the positions of the root joint in the first $P_0$ and last pose $P_{\tau}$, respectively.

% \subsection{Character Simulation}
% During runtime, we first compute desired gait $G_{des}$ using gait generation method described in Section~\ref{sec:gaitGeneration}. Next, we compute collision-free trajectories and update the position of the agents in the ground plane. We retarget the generated gait $G_{des}$ to the avatar of the virtual agent using Unity's skeleton retargeting~\cite{skeletonRetargeting} and update the positions of the agent's joints in the virtual world using the joint positions from $G_{des}$. We use the emotion-based gazing behaviors to update the neck joint's flexion and rotation angles. The resultant virtual agents are then rendered to an HMD.

